Investigating the Benefits of Nonlinear Action Maps in Data-Driven Teleoperation

As robots become more common for both able-bodied individuals and those living with a disability, it is increasingly important that lay people be able to drive multi-degree-of-freedom platforms with low-dimensional controllers. One approach is to use state-conditioned action mapping methods to learn mappings between low-dimensional controllers and high DOF manipulators -- prior research suggests these mappings can simplify the teleoperation experience for users. Recent works suggest that neural networks predicting a local linear function are superior to the typical end-to-end multi-layer perceptrons because they allow users to more easily undo actions, providing more control over the system. However, local linear models assume actions exist on a linear subspace and may not capture nuanced actions in training data. We observe that the benefit of these mappings is being an odd function concerning user actions, and propose end-to-end nonlinear action maps which achieve this property. Unfortunately, our experiments show that such modifications offer minimal advantages over previous solutions. We find that nonlinear odd functions behave linearly for most of the control space, suggesting architecture structure improvements are not the primary factor in data-driven teleoperation. Our results suggest other avenues, such as data augmentation techniques and analysis of human behavior, are necessary for action maps to become practical in real-world applications, such as in assistive robotics to improve the quality of life of people living with w disability.

==> theory.tex <==
\section{Soft Reversibility over Trajectories}
\label{sec:theory}

This section provides bounds on trajectory-wise soft reversibility which accounts for the changing actions over several time steps. We essential show that by reversing the induced vector field of the dynamical system given an action sequence, we are able to return to a previously visited state along that field in the reverse direction. Our analysis is similar to the error analysis of Eulers method and our proofs use standard results on solutions to initial value problems \cite{stuart2009dynamicalsystems}. All proofs are in the appendix.

%Our results on \textit{trajectory soft reversibility} provides information on how one can expect a data-driven interface to behave during deployment. Reversibility is particularly useful as users often expect to be able to undo mistakes when operating a robot. By bounding reversibility, our research provides theoretical guarantees as opposed to only experimental evidence on the behavior of the action mapping function.   

We first show that in a continuous time system, any arbitrary function $f(x(t), a(t))$ can return to the exact initial state $x(0)$. Throughout this section, we define the robotic state $x(t)$ to be the joint configurations of the robot. The actions $a(t)$ are inputs from a policy in a bounded symmetrical domain $a \in [-c, c]^{n}$ for some constant $c \in \mathbf{R}^{+}$. The action map follows the dynamics of Equation~\ref{eqn:dynamicalsystem}. $f$ is Lipschitz continuous for some constant $L$, and is an odd function in actions (i.e. $f(x(t), -a(t)) = -f(x(t), a(t))$). 


\begin{theorem}[Trajectory Reversibility] \label{thm:trajectory_reversibility}
In the interval $0 \leq t \leq 1$ following $f$ Equation~\ref{eqn:dynamicalsystem}, and assuming that $a(t+1) = -a(t-1)$,  we have $x(2- t) = x(t)$.
\end{theorem}


This result reverses the dynamics' gradient flow induced by the user actions' sequence. The theorem suggests that as the sampling rate increases, we expect our action map to get closer to a previously visited state. Even though the movements may change with a state-dependent action map, this result shows that it's possible to perfectly return to a state when doing the opposite action sequence!

\subsection{Reversing with Discretization Error }
Unfortunately, discretization errors cause trajectories to deviate from any initial state when actions are reversed. We account for discretization by bounding the distances from an initial state over a trajectory. We assume that $||f(s, a)|| \leq M$ where $M$ is some maximum action because $a$ is bounded. This is a reasonable assumption as robot joints exist on a bounded space, and we user actions must be bounded at deployment. 

\begin{theorem}[Trajectory Soft Reversibility]
    Suppose there is an odd and bounded function $f(x(t), a(t))$ that is Lipschitz continuous $||f(x(t), a(t)) - f(x'(t), a(t))|| \leq L ||x(t) - x'(t)||$. For points $x_T(k) = x(0) + \sum_{i=0}^{k-1}f(x_T(i), a_T(i))$ such that $ a_T(T+k) = -a_T(T -k)$, then we have $||x_T(0) - x_T(2T)|| \leq \nu M [\exp^{TL\nu} - 1]$
\end{theorem}

A consequence of the above theorem is that one can make specifications on the action mapping during training and at deployment. For example, we can find a hypothetical   sampling rate $\nu$ to guarantee some specified maximal error induced by the action map. Our result would also suggest that generally neary by states are easier to reverse, aligning with previous results and intuition. 

Unfortunately, we found in our experiments that even when trained to be reversible, often autoencoder models do not perfectly reverse actions, often having residual $\epsilon$ of the inverse action $-a$. We add a corollary to our soft reversibility proof which accounts for this residual error. 

\begin{corollary}[Residual Inversing Actions]
    Suppose that $f(x, a)$ is such that $f(x, -a) = -f(x, a) + \epsilon$ is some bounded residual error $||\epsilon|| \leq E$. Then 
    \begin{equation}
        ||x_T(0) - x_T(2T)|| \leq (\nu M + \frac{E}{L}) [\exp^{TL\nu} - 1]
    \end{equation}
\end{corollary}

This provides insight that a typical end-to-end encoder is, at least by our analysis, inappropriate for teleoperation settings. Reducing the residual requires increasing model capacity and data coverge of the tasks interactions. If the neural network is designed to encode reversibility by design, this issue is mitigated directly eliminating any issue of issues in reversed actions. 


